gen2Out: Detecting and Ranking Generalized Anomalies

In a cloud of m-dimensional data points, how would we spot, as well as rank, both single-point- as well as group- anomalies? We are the first to generalize anomaly detection in two dimensions: The first dimension is that we handle both point-anomalies, as well as group-anomalies, under a unified view -- we shall refer to them as generalized anomalies. The second dimension is that gen2Out not only detects, but also ranks, anomalies in suspiciousness order. Detection, and ranking, of anomalies has numerous applications: For example, in EEG recordings of an epileptic patient, an anomaly may indicate a seizure; in computer network traffic data, it may signify a power failure, or a DoS/DDoS attack. We start by setting some reasonable axioms; surprisingly, none of the earlier methods pass all the axioms. Our main contribution is the gen2Out algorithm, that has the following desirable properties: (a) Principled and Sound anomaly scoring that obeys the axioms for detectors, (b) Doubly-general in that it detects, as well as ranks generalized anomaly -- both point- and group-anomalies, (c) Scalable, it is fast and scalable, linear on input size. (d) Effective, experiments on real-world epileptic recordings (200GB) demonstrate effectiveness of gen2Out as confirmed by clinicians. Experiments on 27 real-world benchmark datasets show that gen2Out detects ground truth groups, matches or outperforms point-anomaly baseline algorithms on accuracy, with no competition for group-anomalies and requires about 2 minutes for 1 million data points on a stock machine.

==> 030method.tex <==
\begin{table}[]
	\centering
	\caption{ Table of symbols.\label{tab:symbols}}
	
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{r l}
			\toprule
			Symbol & Definition \\
			\midrule
			$X = \{ \bs{x_i}\}$ & set of observations where $\bs{x_i} \in \mathrm{R}^m$ for $i \in 1, 2, \dots n$\\
			$s(.)$ & anomaly score function for an outlier detector\\
			$h(\bs{x})$ & path length for instance $\bs{x}$ as it traverses a randomized tree\\
			$\mathbb{E}[h(\bs{x})]$ & path length averaged over the ensemble\\
			$H(n)$ & depth estimation function for a randomized tree containing \\
			& $n$ observations\\
			\bottomrule
	\end{tabular}}	
\end{table}

1. Sampled dataset 3 times (2\^(n), 2\^(n+1), 2\^(n+2)) and train the full-grown IF to get the most frequent depth
2. Use n and the most frequent depths to fit linear regression
3. Train a IF with all data and fix depth 8, and without sampling for each base estimator


Our goal is to design a principled, universal anomaly detector that allows for score comparison across point-cloud datasets, and we present the proposed \method. 
\begin{iprob}
	Given multiple point-cloud datasets, find the outliers in each dataset, and then report the most anomalous points across all datasets.
\end{iprob}
Motivated by our epilepsy application, we aim to apply it to draw attention to anomalous periods in a multivariate time series data, and to point to variables that characterize the flagged anomalous period. We are given $\mathbb{T} = \{ \mathcal{T}_i\}, i= 1, 2, \dots$ a set of multivariate time series. Each time series $\mathcal{T} \in  \mathbb{T}$ consists of signal measurements $\bs{x_t} = (x_{t1} , \dots, x_{tM} )$ across $M$ variables (electrode channels in seizure data) at each time step $t=1, 2, . . . , T$. To find anomalous patterns that occur in multivariate time series $\mathcal{T}$, we divide time-series data $\mathcal{T}$ into subsequence $S_j$ according to the sliding window size $K$. We characterize each univariate series of length $K$ with several features such that each univariate series becomes a $m$-dimensional point. In particular, each univariate series in the multivariate time series is summarized by a set of features extracted from its statistical properties such as first four moments, and each subsequence $S_j$ is transformed into a point cloud data matrix $X_j \in \mathrm{R}^{M \times m}$. We then apply \method (details to follow next) to each data matrix $X_j$ and record the anomalousness of each (electrode channel) variable $\in 1, \dots, M$ for each period of time (window size $K$). The key property of \method is that it obeys the axioms that an ideal detector should follow enabling us to reason about the anomalousness of each time period and the anomalousness of each variable within a time period by comparing their respective anomaly scores. Therefore, each time period is now represented by an anomaly score vector through which we can draw attention of the domain experts to anomalous time periods.
% In this section we present the proposed method,
% we analyze it and provide the reader with several interesting -at least in our opinion-
% observations. 
\begin{algorithm2e}[!h]
	% \SetAlgoVlined
	\SetAlgoLined
	% \SetNoLine
	\LinesNumbered
	\KwData{A data matrix $X$, number of \tree estimators \texttt{numTrees}, \tree depth limit \texttt{depthLimit}}
	\KwResult{Depth estimation function $H(\cdot)$ and \tree ensemble}
	Initialize $Y$ and $Z$\;
	\tcc{Estimating the function $H(\cdot)$}
	
	\For{$i = n_1, n_1 + 1 \dots$}{\tcp*{a small number $n_1$ e.g. 10}
		Draw $X_{s} \subset X \text{ s.t. } |X_{s}| = 2^i$ \;
		% Randomly sample $2^i$ data points $X^{'}$ from $X$\;
		$F_s \leftarrow$ \texttt{Construct\tree}($X_s$, $\infty$)\;
		Compute depth distribution of data points in $X_s$ using  $F_s$\;
		Identify the mode of the distribution and add it into $Z$\;
		Add $i$ to $Y$\;
	}
	$H(\cdot) \leftarrow$ Fit linear regression $Y$ and $Z$\;
	\tcc{Construct the ensemble of \tree}\;
	\For{t = 1 to \texttt{numTrees}}{
		\texttt{ensemble} $\leftarrow$  \texttt{ensemble} $\cup$ \texttt{Construct\tree}($X$, \texttt{depthLimit})\;
	}
	\caption{\method-Fit \label{algo:fit}}
\end{algorithm2e}
\subsection{\method Algorithm}
Given the observations $X = \{ \bs{x_1}, \dots, \bs{x_M} \}$ where $\bs{x_i} \in \mathrm{R}^m$, \method's goal is to detect and assign anomaly score to outlier points. \method uses an ensemble of randomized tree \tree ({\S\ref{subsec:insights}}) that recursively partition instances in $X$. Random tree partitioning is repeated until a tree depth limit is reached or each {\em leaf} contains exactly one instance. As evidenced in prior works, the random trees induce shorter path lengths (number of steps from root node to leaf node while traversing the tree) for anomalous observations since the instances that deviate from other observations are likely to be partitioned early. Therefore, a shorter average path length from the ensemble would likely indicate an anomalous observation. Anomaly detection is essentially a ranking task where the rank of an instance indicates its relative degree of anomalousness. We next design anomaly score function for our algorithm to facilitate ranking of observations.\\
% \vspace{0.05in}
% \subsubsection{Anomaly Score}
\begin{algorithm2e}[!h]
	% \SetAlgoVlined
	\SetAlgoLined
	% \SetNoLine
	\LinesNumbered
	\KwData{A data matrix $X$, \texttt{depthLimit}, \texttt{currDepth:0}}
	\KwResult{\tree}
	Initialize \tree\;
	\uIf{\texttt{depthLimit} is not reached \text{or} $|X| \leq1$}{
		return \texttt{leaf}\{$X$\}
	}
	\Else{sample an attribute from the list of attributes in $X$\;
		randomly select an attribute value for the selected attribute\;
		$X_l\leftarrow$ \texttt{filter} observations that are less than compared to sampled attribute-value pair\;
		$X_r\leftarrow$ \texttt{filter} observations that are greater than compared to sampled attribute-value pair\;
		\texttt{left}  $\leftarrow$ \texttt{Construct\tree}($X_l$,\texttt{depthLimit}, \texttt{currDepth + 1})\;
		\texttt{right} $\leftarrow$ \texttt{Construct\tree}($X_r$,\texttt{depthLimit}, \texttt{currDepth + 1})
		
		return \texttt{internalNode}\{\texttt{left}, \texttt{right}, \{sampled attribute-value pair\}\}
		
	}
	\caption{\texttt{Construct \tree} \label{algo:tree}}
\end{algorithm2e}
\noindent {\bfseries Proposed Anomaly Score.~}
We construct anomaly score using the path length $h(\bs{x})$ for each instance $\bs{x}$ as it traverses an \tree.  The path length for $\bs{x}$ is $h(\bs{x}) = h_{leaf} + H(n_{leaf}) \mathbbm{1}\{{n_{leaf} > 1}\}$, where  $h_{leaf} $ is
the number of edges $\bs{x}$ traverses from \emph{root} to \emph{leaf} node containing $n_{leaf}$ points in an \tree, $\mathbbm{1}\{{n_{leaf} > 1}\}$ evaluates if the leaf node contains more than one instance in which case we estimate the depth using $H(n_{leaf})$. We normalize $h(\bs{x})$ by the average tree height $H(n)$ (height of \tree containing $n$ observations) for the \tree ensemble to produce an anomaly score $s(\bs{x}, n)$ for a given observation $\bs{x}$. Referring to the insights we presented in Section \S\ref{subsec:insights}, we estimate the data dependent $H(\cdot)$ since the tree depth grows linearly with the number of observations (in $log_2$) in the tree (see Figure~\ref{fig:depthdist}). Following the \llshort{} property, we fit a linear function to estimate the expected depth for a given number of samples in the \tree (see Figure~\ref{fig:depthdist}). The slope of the linearity is characterized by underlying data distribution, though each distribution follows a linear growth. The score function is
\begin{equation}
    s(\bs{x}, n) = 2^{- \frac{\mathrm{E}[h(\bs{x})]}{H(n)}}
\end{equation}
where $\mathrm{E}[h(\bs{x})]$ is the average path length of observation $\bs{x}$ in the \tree ensemble, $n$ is number of data points used to construct each \tree, and $H(n)$ is the function for estimating depth of the tree given in Eq.~\ref{eq:hn}.\\
%\begin{equation}
%	\label{eq:hn}
%    H(n) = w_0 + w_1 log_2(n)
%\end{equation}
%where $w_0$ and $w_1$ are parameters that we estimate for each data distribution.\\

\noindent {\bfseries \method Parameter Fitting.~} \method is a \tree ensemble that is constructed by recursively partitioning the given set of observations $X$ until a depth limit is reached or {\em leaf} nodes contain exactly one instance. The algorithm for training \method is provided in Algorithms~\ref{algo:fit} and \ref{algo:tree}.\looseness=-1\\
\begin{algorithm2e}[]
% \SetAlgoVlined
\SetAlgoLined
% \SetNoLine
\LinesNumbered
\KwData{A data matrix $X$, \tree ensemble}
\KwResult{Anomaly scores \texttt{scores} for observations in $X$}
Initialize \texttt{depths}\;
Initialize \texttt{scores}\;
Initialize \texttt{numSamplesInLeaf}\;
$n \leftarrow$ \texttt{numSamplesIn\tree}\;
\For{$\bs{x} \in X$}{
    \texttt{depths} $\leftarrow$ \texttt{depths} $\cup$ compute path-lengths for $\bs{x}$\;
    \texttt{numSamplesInLeaf} $\leftarrow$ \texttt{numSamplesInLeaf} $\cup$ compute number of samples in \texttt{leaf} where traversal of $\bs{x}$ terminated\;
}
\For{depth $\in$ \texttt{depths}, $l \in$ \texttt{numSamplesInLeaf}}{
    $h = $depth$ + H(l)$\;
    $s = 2^{\frac{-h}{H(n)}}$\;
    \texttt{scores} $\leftarrow$ \texttt{scores} $\cup~ s$\;
}
return \texttt{scores}\;
\caption{\method-Predict \label{algo:predict}}
\end{algorithm2e}

\noindent {\bfseries \method Scoring.~} To assign anomaly scores to the instances in a data matrix $X$, the expected path length $\mathrm{E}(h(\bs{x}))$ for each instance $\bs{x} \in X$. $\mathrm{E}(h(\bs{x}))$ is estimated by averaging the path length after tree traversal through each \tree in \method ensemble. We outline the steps to assign anomaly score to a data point using \method in Algorithm~\ref{algo:predict}.
% 
%  
% Table~\ref{tab:dfn} gives the list of symbols we use.

% \notice{Give table of symbols and dfns}

% \begin{table}[htbp]
% \begin{center}


% \begin{tabular}{|c|c|}
% \hline  
% Symbols & Definitions \\ 
% \hline
% $G$  & a graph \\ 
% \hline  
% $A$  &  adjacency matrix\\ 
% \hline 
% \end{tabular} 
% \caption{Symbols and Definitions \label{tab:dfn}}
% \end{center}
% \end{table}

==> 080listOfToDo.tex <==
\todototoc
\listoftodos

==> makefile <==
MAIN=paper
FINAL= final
SRC= 				\
	000abstract.tex		\
	010introduction.tex		\
	020background.tex		\
	021preliminaries.tex		\
	030method.tex		\
	031method.tex		\
	040experiment.tex		\
	060conclusion.tex		\
	070appendix.tex		\
	080listOfToDo.tex		\
	dfn.tex

pdf: $(MAIN).pdf

final: $(FINAL).pdf

$(FINAL).pdf: $(MAIN).tex mkfinal.pl
	perl mkfinal.pl $(MAIN).tex > $(FINAL).tex
	pdflatex $(FINAL).tex
	bibtex $(FINAL)
	pdflatex $(FINAL).tex
	pdflatex $(FINAL).tex

$(MAIN).pdf: $(MAIN).tex $(SRC)
	pdflatex $(MAIN)
	bibtex $(MAIN)
	pdflatex $(MAIN)
	pdflatex $(MAIN)

clean:
	\rm -f *.log *.bbl *.blg *.out *.aux
	\rm -f *.toc
	\rm -f $(MAIN).synctex.gz

spotless: clean
	\rm -f $(MAIN).pdf
	\rm -f $(FINAL).pdf $(FINAL).tex

